Rare Tokens Degenerate All Tokens: Improving Neural Text Generation via Adaptive Gradient Gating for Rare Token Embeddings

Recent studies have determined that the learned token embeddings of large-scale neural language models are degenerated to be anisotropic with a narrow-cone shape. This phenomenon, called the representation degeneration problem, facilitates an increase in the overall similarity between token embeddings that negatively affect the performance of the models. Although the existing methods that address the degeneration problem based on observations of the phenomenon triggered by the problem improves the performance of the text generation, the training dynamics of token embeddings behind the degeneration problem are still not explored. In this study, we analyze the training dynamics of the token embeddings focusing on rare token embedding. We demonstrate that the specific part of the gradient for rare token embeddings is the key cause of the degeneration problem for all tokens during training stage. Based on the analysis, we propose a novel method called, adaptive gradient gating (AGG). AGG addresses the degeneration problem by gating the specific part of the gradient for rare token embeddings. Experimental results from language modeling, word similarity, and machine translation tasks quantitatively and qualitatively verify the effectiveness of AGG.

==> sections/C.Ablation_raregroup.tex <==
\section{Ablation Study about AGG} \label{appenC}
In this section, we present the ablation studies about AGG. In our method, AGG, we introduce two gate vectors, $\textbf{g}_1$, and $\textbf{g}_2$, to handle the gradient for rare and very rare token embeddings. We conduct experiments on these gate vectors. Table \ref{table_abl} presents the results of the ablation studies compared with the MLE and AGG. When $\textbf{g}_1$ is excluded from AGG (denoted as 'no $\textbf{g}_1$'), Uniq and $I(\textbf{W})$ decreased significantly, because $\textbf{g}_1$ is the key component for the gradient gating. When $\textbf{g}_2$ is excluded from AGG (denoted as 'no $\textbf{g}_2$'), Uniq and $I(\textbf{W})$ slightly decrease. Accordingly, we notice that $\textbf{g}_2$ is important for the gating of gradients fort the very rare token embeddings.

Also, we present the analysis about rare token grouping method of AGG. Figure \ref{fig_raregroupsize} presents the size of the rare token group during initial 1k training steps when the model is trained with WikiText-103 dataset. As presented in the figure, rare group size fluctuate wildly at the initial training stage. We expect for this grouping method to determine an optimal rare token group for the current training step. Table \ref{table_abl_grouping} presents the results of ablation study about dynamic grouping. To except dynamic grouping from AGG, we fixed the rare token group after 1 epoch. For this static grouping AGG method, Next-token diversity(Uniq) and the isotropy of the token embedding space($I(\textbf{W})$ perform worse than dynamic grouping AGG.

\begin{table}[t]
\centering
\begin{tabular}{l||ccc}
\hline
\toprule
\multirow{2}{*}{\textbf{Methods}} &
\multicolumn{3}{c}{$\mathbf{I(W)}$$\uparrow$} \\ 
 & Freq & Med & Rare \\
\hline
MLE & 0.51 & 0.33 & 0.278  \\
AGG & \textbf{0.702} & \textbf{0.714} & \textbf{0.813} \\

\bottomrule
\end{tabular}
\caption{Experimental results about $\mathbf{I(W)}$ for each token group in WikiText-103 language modeling task comparing MLE baseline and AGG.}
\label{table_i_mle}
\end{table}

\begin{table}[t]
\centering
\begin{tabular}{l||ccc}
\hline
\toprule
\multirow{2}{*}{\textbf{Methods}} &
\multicolumn{3}{c}{$\mathbf{I(W)}$$\uparrow$} \\ 
 & Freq & Med & Rare \\
\hline
UL & 0.533 & 0.351 & 0.293  \\
UL + AGG & \textbf{0.731} & \textbf{0.626} & \textbf{0.696} \\

\bottomrule
\end{tabular}
\caption{Experimental results about $\mathbf{I(W)}$ for each token group in WikiText-103 language modeling task comparing UL baseline and UL + AGG.}
\label{table_i_ul}
\end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{l||c|c|c}
% \hline
% \toprule
% \textbf{Method} & \textbf{PPL}$\downarrow$ & \textbf{Uniq}$\uparrow$ & $\mathbf{I(W)}$$\uparrow$  \\
% \hline
% MLE & 15.51 & 13143 & 0.377 \\
% AGG & 15.51 & 13737 & 0.813 \\
% no $\textbf{g}_1$ & 15.48 & 13018 & 0.367 \\
% no $\textbf{g}_2$ & 15.51 & 13682 & 0.701 \\
% \bottomrule
% \end{tabular}
% \caption{Ablation study on gating vector of AGG.}
% \label{table_abl}
% \end{table}

% \begin{table}
% \centering
% \begin{tabular}{l||c|c|c}
% \hline
% \toprule
% \textbf{Method} & \textbf{PPL}$\downarrow$ & \textbf{Uniq}$\uparrow$ & $\mathbf{I(W)}$$\uparrow$  \\
% \hline
% MLE & 15.51 & 13143 & 0.377 \\
% AGG & 15.51 & 13737 & 0.813 \\
% static AGG & 15.55 & 13614 & 0.752 \\
% \bottomrule
% \end{tabular}
% \caption{Ablation study about dynamic grouping of AGG.}
% \label{table_abl_grouping}
% \end{table}

% \begin{figure}[t]
%      \centering
%      \includegraphics[width=0.45\textwidth]{sections/figs/rare_group_size.pdf}
%      \caption{Size of the rare token group during initial 1k steps of training with WikiText-103 dataset.}
%      \label{fig_raregroupsize}
% \end{figure}
